A Delphi Study on the Adaptation of SCRUM Practices to Remote Work

This study explores how Scrum practices were adjusted for remote and hybrid work during and after the COVID-19 pandemic, using a Delphi study with Scrum Masters to gather expert insights. Preliminary key findings highlight communication as the primary challenge, leading to adjustments in meeting structures, information-sharing practices, and collaboration tools. Teams restructured ceremonies, introduced new meetings, and implemented persistent information-sharing mechanisms to improve their work.

==> Tables/experts.tex <==
\begin{table}[!htp]\centering
\caption{Panel of Experts}
\label{tab:experts}
\scriptsize
\begin{tabular}{|p{5cm}|p{5cm}|p{5cm}|}
\hline
\multicolumn{3}{|c|}{\textbf{Experts Profile}} \\ \hline
\textbf{Category} & \textbf{Subcategory} & \textbf{Details} \\ \hline

\multirow{2}{*}{Gender} 
& Male & 5 experts \\ \cline{2-3}
& Female & 3 experts \\ \hline

\multirow{2}{*}{Highest Educational Level}
& Bachelor Degree & 1 expert \\ \cline{2-3}
& Post-graduate Diploma & 7 experts \\ \hline

\multirow{2}{*}{Software Industry Experience}
& 5 - 10 Years & 5 experts \\ \cline{2-3}
& 10+ Years & 3 experts \\ \hline

\multirow{2}{*}{Scrum Master Experience}
& 5 - 10 Years & 4 experts \\ \cline{2-3}
& 10+ Years & 4 experts \\ \hline

\multirow{2}{*}{Current Work Environment}
& Hybrid & 1 expert \\ \cline{2-3}
& Remote & 7 experts \\ \hline

\multirow{2}{*}{Underrepresented Group in SE}
& Black Person & 1 expert \\ \cline{2-3}
& LGBTQIA+ Individual & 1 expert \\ \hline

\end{tabular}
\end{table}

